LENS: A Learnable Evaluation Metric for Text Simplification

Training learnable metrics using modern language models has recently emerged as a promising method for the automatic evaluation of machine translation. However, existing human evaluation datasets for text simplification have limited annotations that are based on unitary or outdated models, making them unsuitable for this approach. To address these issues, we introduce the SimpEval corpus that contains: SimpEval_past, comprising 12K human ratings on 2.4K simplifications of 24 past systems, and SimpEval_2022, a challenging simplification benchmark consisting of over 1K human ratings of 360 simplifications including GPT-3.5 generated text. Training on SimpEval, we present LENS, a Learnable Evaluation Metric for Text Simplification. Extensive empirical results show that LENS correlates much better with human judgment than existing metrics, paving the way for future progress in the evaluation of text simplification. We also introduce Rank and Rate, a human evaluation framework that rates simplifications from several models in a list-wise manner using an interactive interface, which ensures both consistency and accuracy in the evaluation process and is used to create the SimpEval datasets.

==> fig/lens_overview.tex <==
\begin{figure*}[t!]

\begin{center}
\includegraphics[width=0.99\linewidth]{img/figure2_overview.pdf}
\end{center}
\vspace{-3pt}
\caption{\yd{TO-DO}}
\vspace{-3pt}
\label{fig:figure_2}
\end{figure*}

==> tab/human_eval_2022_data_stats.tex <==
\begin{table}[!ht]
\centering
{\renewcommand{\arraystretch}{1.0}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc}\toprule
Stats & \likertdatasetname\textsubscript{\textsc{2022}} & \dadatasetname\textsubscript{\textsc{2022}}  & \datasetnameSecond \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
Number of systems & 6 & 6 & 6 \\
Number of instances & 360 & 360 & 360 \\
Number of ratings per instance & 3 & 3 & 3 \\
\midrule
Inter-annotator agreement & \\
Time per annotation & \\
\bottomrule
\end{tabular}
}}
\caption{} 
\label{tab:human_eval_asset_data_stats}
\end{table}

==> tab/human_eval_asset_data_stats.tex <==
\begin{table}[!t]
\centering
{\renewcommand{\arraystretch}{1.0}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc}\toprule
Stats & \likertdatasetname\textsubscript{\textsc{ASSET}} & \dadatasetname\textsubscript{\textsc{ASSET}}  & \datasetnameFirst\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
Number of systems & \\
Number of instances & \\
Number of ratings per instance & \\
Year of the best system & \\
Include transformer models? & \\
Include human simplifications? & \\
\midrule
Inter-annotator Agreement & \\
\bottomrule
\end{tabular}
}}
\caption{} 
\label{tab:human_eval_asset_data_stats}
\end{table}

==> tab/human_eval_comparison.tex <==
\begin{table}[t!]
\small
\centering
\begin{tabular}{lccc|c}\toprule
& \textbf{OS} & \textbf{RR} & \textbf{CS} & \textbf{Krippendorff's $\alpha$} \\
\midrule
\likertdatasetname & &  & &  0.23\\
\dadatasetname & &  & \checkmark & 0.25 \\
\datasetnameSecond & \checkmark & \checkmark & \checkmark &\textbf{0.32} \\
\bottomrule
\end{tabular}
\caption{Comparison of different text simplification human evaluation methods. \textbf{OS}: One Score, \textbf{RR}: Relative Ranking, \textbf{CS}: Continuous Scale.}
\vspace{-0.5cm}
\label{tab:human_eval_comparison}
\end{table}

==> tab/iaa_results.tex <==
\begin{table}[t!]
\small
\centering
\begin{tabular}{lc}\toprule
& Krippendorff's $\alpha$ \\
\midrule
\likertdatasetname &  0.23\\
\dadatasetname & 0.25 \\
\datasetnameSecond & \textbf{0.32} \\
\bottomrule
\end{tabular}
\caption{Inter-annotator agreement of human ratings collected using different human evaluation methods.\yd{explain why the score is low.}} 
\label{tab:iaa_results}
\end{table}

==> tab/mrt_mbr_big.tex <==
\begin{table*}[t!]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
 & \textbf{Model} & \textbf{BLEU} $\uparrow$  &  \textbf{SARI} $\uparrow$ & \textbf{BERTScore} $\uparrow$ & \textbf{\metricname} $\uparrow$ &  \textbf{sBLEU} $\downarrow$ & \textbf{Human} $\uparrow$  \\
\midrule
MLE$_{beam=10}$ & T5$_{base}$  & 44.4 & 47.5 & \textbf{94.7} & 61.0 & 70.7 &  68.71 \\
MLE$_{beam=100}$ & T5$_{base}$  & 42.6 & 42.6 & 94.3 & 57.6 & 68.1 & -- \\
MLE$_{beam=100}$ & T5$_{3B}$  &  39.7 & 42.5 & 94.0 & 53.4 & 65.4 & -- \\
MLE$_{beam=100}$ & T5$_{11B}$  &  35.8 & 44.7 & 93.2 & 59.2 & 51.1 & --\\
\midrule
\multicolumn{7}{l}{\textit{Minimum Risk Training (MRT)}} \\
\midrule
BLEU & T5$_{base}$  & \textbf{45.1} & 47.3 & \textbf{94.7} & 60.5 & 71.3 &  68.33 \\
SARI & T5$_{base}$  &  43.4 & 48.5 & 94.5 & 63.2 & 68.1 & \underline{70.86} \\
BERTScore & T5$_{base}$ & 44.0 & 48.4 & \underline{94.6} & 62.1 & 67.8 & 70.32 \\
\metricname & T5$_{base}$  & 42.6 & 47.4 & 94.5 & \underline{63.9} & \underline{67.1} & 68.89\\
\midrule
\multicolumn{7}{l}{\textit{Minimum Bayes Risk Decoding (MBR)}} \\
\midrule
BLEU & T5$_{base}$  & \underline{44.8} & 48.3 & 94.4 & 60.4 & 74.1 & 66.19 \\
SARI  &  T5$_{base}$  &43.9 & \textbf{49.6} & 94.5 & 59.3 & 75.5 & 64.31 \\
BERTScore & T5$_{base}$  & 44.3 & 48.3 & \underline{94.6} & 61.1 & 72.1 & 66.79 \\
\metricname  & T5$_{base}$  & 43.2 & \underline{49.5} & \textbf{94.7} & \textbf{73.1} & \textbf{61.8} & \textbf{72.80} \\
\metricname & T5$_{3B}$  & 42.3 & 47.7 & 94.9  & 72.6 & 55.7 & --  \\
\metricname & T5$_{11B}$  & 36.2 & 46.1 & 93.8 &  74.4 & 44.6 & -- \\
\bottomrule
\end{tabular}
\caption{Evaluation results for minimum risk training (MRT)  and minimum Bayes risk decoding (MBR) on \datasetnameSecond. We report \textbf{\metricname}, BLEU (\textbf{BL}), \textbf{SARI}, BERTScore (\textbf{BS}), self-BLEU (\textbf{sBL}), and average human ratings. MBR with \metricname~ shows the best human evaluation results while making the most number of edits to the input as indicated by its lowest self-BLEU.}
\label{table:mrt_mbr_eval_results}
% \vspace{-1cm}
\end{table*}

==> tab/simpeval_2022.tex <==
\begin{table*}[!htbp]
\small
\centering
\begin{tabular}{lccccccccc}\toprule
 & \multicolumn{4}{c}{\textbf{\likertdatasetname}} & \multicolumn{4}{c}{\textbf{\dadatasetname}}  & \textbf{\datasetnameSecond}\\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10}
 & \textbf{Fluency} & \textbf{Adequacy} & \textbf{Simplicity} & \textbf{Avg.} & \textbf{Fluency} & \textbf{Adequacy} & \textbf{Simplicity} & \textbf{Avg.} & \textbf{Overall} \\ \midrule
Human-1 & 4.69 & 4.46 & 1.36 & 3.50 & 0.094 & 0.132 & \textbf{0.347} & \textbf{0.191} & 0.395\\ 
Human-2 & \textbf{4.72} & 4.48 & \textbf{1.39} & \textbf{3.53}  & \textbf{0.135} & 0.045 & 0.339 & 0.173  & \textbf{0.424}\\
GPT-3.5 (5-shot) & 4.64 & \textbf{4.66} & 1.13 & 3.48 & 0.134 & \textbf{0.247} & 0.108 & 0.163 & 0.280 \\
GPT-3.5 (zero-shot)& 4.63 & 4.56 & 0.91 & 3.37 & -0.060 & 0.208 & -0.261 & -0.036 & -0.025\\
MUSS & 4.40 & 4.11  & 0.86 & 3.12  & -0.265 & -0.429 & -0.330 & -0.342  & -0.333 \\ 
T5-3B & 4.70 & 4.33 & 0.55 & 3.19 & -0.037 & -0.225 & -0.215 & -0.159  & -0.700\\
\bottomrule
\end{tabular}
\caption{Performance by the model in three different human evaluation methods. Both \dadatasetname~and \datasetnameSecond~report z-score. Humans outperform GPT-3.5 in the few-shot setting. \textbf{Bold}: the best. \yd{use raw score}} 
\label{tab:simpeval_2022}
\end{table*}

==> tab/simpeval_asset_analysis.tex <==
\begin{table*}[!htbp]
\small
\centering
{\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccc}\toprule
System & Z-score & Raw & Length & \# Edits & \% Keep & \% New & \% Split\\ \midrule
Human-1 & \cellcolor{teal7}\textcolor{white}{0.877}  & \cellcolor{teal1}{85.85}  & \cellcolor{teal4}{19.51}  & \cellcolor{teal5}\textcolor{white}{3.98}  & \cellcolor{teal3}{65.57}  & \cellcolor{teal6}\textcolor{white}{22.2}  & \cellcolor{teal3}{25.0}  \\ 
Human-2 & \cellcolor{teal7}\textcolor{white}{0.76}  & \cellcolor{teal7}\textcolor{white}{84.28}  & \cellcolor{teal4}{18.55}  & \cellcolor{teal5}\textcolor{white}{4.71}  & \cellcolor{teal2}{59.91}  & \cellcolor{teal7}\textcolor{white}{25.07}  & \cellcolor{teal3}{21.0}  \\ 
Muss & \cellcolor{teal7}\textcolor{white}{0.724}  & \cellcolor{teal7}\textcolor{white}{83.1}  & \cellcolor{teal6}\textcolor{white}{21.28}  & \cellcolor{teal5}\textcolor{white}{4.35}  & \cellcolor{teal3}{66.03}  & \cellcolor{teal1}{26.09}  & \cellcolor{teal4}{35.0}  \\ 
T5 & \cellcolor{teal7}\textcolor{white}{0.709}  & \cellcolor{teal7}\textcolor{white}{83.17}  & \cellcolor{teal7}\textcolor{white}{23.46}  & \cellcolor{teal5}\textcolor{white}{4.06}  & \cellcolor{teal4}{73.2}  & \cellcolor{teal7}\textcolor{white}{25.54}  & \cellcolor{teal5}\textcolor{white}{44.0}  \\ 
Transformer & \cellcolor{teal6}\textcolor{white}{0.437}  & \cellcolor{teal6}\textcolor{white}{78.48}  & \cellcolor{teal4}{19.08}  & \cellcolor{teal3}{2.52}  & \cellcolor{teal3}{66.86}  & \cellcolor{teal5}\textcolor{white}{17.3}  & \cellcolor{teal2}{14.0}  \\ 
Controllable & \cellcolor{teal6}\textcolor{white}{0.355}  & \cellcolor{teal6}\textcolor{white}{77.63}  & \cellcolor{teal6}\textcolor{white}{21.65}  & \cellcolor{teal3}{2.39}  & \cellcolor{teal5}\textcolor{white}{81.75}  & \cellcolor{teal4}{12.22}  & \cellcolor{teal1}{8.0}  \\ 
Simple Wiki & \cellcolor{teal6}\textcolor{white}{0.276}  & \cellcolor{teal6}\textcolor{white}{76.65}  & \cellcolor{teal6}\textcolor{white}{22.47}  & \cellcolor{teal4}{3.7}  & \cellcolor{teal4}{75.19}  & \cellcolor{teal6}\textcolor{white}{21.54}  & \cellcolor{teal1}{0.0}  \\ 
Human-T & \cellcolor{teal6}\textcolor{white}{0.27}  & \cellcolor{teal6}\textcolor{white}{76.71}  & \cellcolor{teal6}\textcolor{white}{21.37}  & \cellcolor{teal4}{3.38}  & \cellcolor{teal4}{75.97}  & \cellcolor{teal5}\textcolor{white}{18.24}  & \cellcolor{teal1}{7.0}  \\ 
Dress & \cellcolor{teal6}\textcolor{white}{0.257}  & \cellcolor{teal6}\textcolor{white}{76.04}  & \cellcolor{teal2}{16.15}  & \cellcolor{teal2}{1.34}  & \cellcolor{teal3}{65.19}  & \cellcolor{teal4}{13.35}  & \cellcolor{teal1}{1.0}  \\ 
Access & \cellcolor{teal5}\textcolor{white}{0.059}  & \cellcolor{teal5}\textcolor{white}{72.52}  & \cellcolor{teal7}\textcolor{white}{23.13}  & \cellcolor{teal4}{3.28}  & \cellcolor{teal5}\textcolor{white}{77.55}  & \cellcolor{teal6}\textcolor{white}{19.49}  & \cellcolor{teal3}{26.0}  \\ 
Copy & \cellcolor{teal5}\textcolor{white}{0.056}  & \cellcolor{teal6}\textcolor{white}{73.41}  & \cellcolor{teal6}\textcolor{white}{22.69}  & \cellcolor{teal1}{0.0}  & \cellcolor{teal1}{100.0}  & \cellcolor{teal1}{0.0}  & \cellcolor{teal1}{0.0}  \\ 
SBMT-SARI & \cellcolor{teal5}\textcolor{white}{0.024}  & \cellcolor{teal5}\textcolor{white}{72.54}  & \cellcolor{teal1}{24.35}  & \cellcolor{teal4}{3.12}  & \cellcolor{teal5}\textcolor{white}{82.14}  & \cellcolor{teal6}\textcolor{white}{21.01}  & \cellcolor{teal1}{0.0}  \\ 
PBMT-R & \cellcolor{teal5}\textcolor{white}{-0.011}  & \cellcolor{teal5}\textcolor{white}{71.82}  & \cellcolor{teal7}\textcolor{white}{23.31}  & \cellcolor{teal3}{2.31}  & \cellcolor{teal6}\textcolor{white}{85.04}  & \cellcolor{teal5}\textcolor{white}{15.05}  & \cellcolor{teal1}{2.0}  \\ 
Edit-NTS & \cellcolor{teal5}\textcolor{white}{-0.07}  & \cellcolor{teal5}\textcolor{white}{70.59}  & \cellcolor{teal6}\textcolor{white}{21.87}  & \cellcolor{teal2}{1.89}  & \cellcolor{teal4}{72.64}  & \cellcolor{teal5}\textcolor{white}{18.45}  & \cellcolor{teal1}{7.0}  \\ 
LSTM & \cellcolor{teal5}\textcolor{white}{-0.157}  & \cellcolor{teal5}\textcolor{white}{68.75}  & \cellcolor{teal3}{17.41}  & \cellcolor{teal3}{2.21}  & \cellcolor{teal3}{65.99}  & \cellcolor{teal4}{14.62}  & \cellcolor{teal1}{1.0}  \\ 
SEMoses & \cellcolor{teal4}{-0.418}  & \cellcolor{teal4}{65.32}  & \cellcolor{teal7}\textcolor{white}{23.68}  & \cellcolor{teal4}{3.56}  & \cellcolor{teal5}\textcolor{white}{80.16}  & \cellcolor{teal5}\textcolor{white}{16.37}  & \cellcolor{teal1}{66.0}  \\ 
UNTS & \cellcolor{teal4}{-0.507}  & \cellcolor{teal4}{63.69}  & \cellcolor{teal4}{18.71}  & \cellcolor{teal3}{2.01}  & \cellcolor{teal5}\textcolor{white}{78.62}  & \cellcolor{teal3}{8.68}  & \cellcolor{teal1}{0.0}  \\ 
UNMT & \cellcolor{teal4}{-0.565}  & \cellcolor{teal4}{61.9}  & \cellcolor{teal6}\textcolor{white}{21.99}  & \cellcolor{teal4}{3.58}  & \cellcolor{teal6}\textcolor{white}{86.38}  & \cellcolor{teal3}{8.11}  & \cellcolor{teal1}{0.0}  \\ 
RM+EX+LS+RO & \cellcolor{teal4}{-0.578}  & \cellcolor{teal4}{61.67}  & \cellcolor{teal4}{19.35}  & \cellcolor{teal4}{2.97}  & \cellcolor{teal3}{69.42}  & \cellcolor{teal5}\textcolor{white}{17.84}  & \cellcolor{teal1}{0.0}  \\ 
Hybrid & \cellcolor{teal3}{-0.767}  & \cellcolor{teal3}{58.47}  & \cellcolor{teal1}{13.53}  & \cellcolor{teal5}\textcolor{white}{4.06}  & \cellcolor{teal1}{47.55}  & \cellcolor{teal6}\textcolor{white}{19.21}  & \cellcolor{teal1}{1.0}  \\ 
Scramble words & \cellcolor{teal1}{-1.733}  & \cellcolor{teal1}{41.05}  & \cellcolor{teal6}\textcolor{white}{22.69}  & \cellcolor{teal1}{6.81}  & \cellcolor{teal7}\textcolor{white}{99.7}  & \cellcolor{teal1}{0.3}  & \cellcolor{teal3}{26.0}  \\ 
\bottomrule
\end{tabular}
}}
\caption{} 
\label{tab:all_systems}
\end{table*}
